Diversity and Exploration in Social Learning

In consumer search, there is a set of items. An agent has a prior over her value for each item and can pay a cost to learn the instantiation of her value. After exploring a subset of items, the agent chooses one and obtains a payoff equal to its value minus the search cost. We consider a sequential model of consumer search in which agents' values are correlated and each agent updates her priors based on the exploration of past agents before performing her search. Specifically, we assume the value is the sum of a common-value component, called the quality, and a subjective score. Fixing the variance of the total value, we say a population is more diverse if the subjective score has a larger variance. We ask how diversity impacts average utility. We show that intermediate diversity levels yield significantly higher social utility than the extreme cases of no diversity (when agents under-explore) or full diversity (when agents are unable to learn from each other) and quantify how the impact of the diversity level changes depending on the time spent searching.

==> valuemodel.tex <==
%!TEX root =  main.tex

\subsection{Proof of Theorem~\lowercase{\ref{thm:value}}}
\label{sec:value}

We define $M(\sigma,\tau)$ to be maximum expected quality over the items which have been searched at the end of round $\tau$. The expectation is taken over the distribution given the history of first $\tau$ rounds. This is like an analog of the $M(\sigma,T)$ in the quality model. Notice that now $M(\sigma,\tau)$ is a random variable and is not the highest quality of items which have been searched because $M(\sigma,\tau)$ is based on the bayesian update of the agent in round $\tau+1$, not the actual quality. This is the main technical difficulty behind the value model.

To prove Theorem~\lowercase{\ref{thm:value}}, we show two lemmas, Lemma \ref{lem:utilitylb} which shows that the expected average utility can be bounded in terms of $M(\sigma,\tau)$ and Lemma \ref{lem:qualitylb} which gives a bound on $M(\sigma,\tau)$.


\begin{lemma}
\label{lem:utilitylb}
For any $0 < \sigma < 1$,  We have $A(\sigma,T) \geq \E[ \max(M(\sigma,T/2)-c, 0 )]/2$. 
\end{lemma}

\begin{proof}
Consider the following strategies of the agents:
\begin{enumerate}
\item For agents in round $1,...,T/2$, use Pandora's rule.
\item For agents in round $T/2+1,...,T$, if $M(\sigma,T/2) \geq c$ explore and pick the item with expected quality $M(\sigma,T/2)$ at the end of round $T/2$. Otherwise leave with utility 0.  
\end{enumerate}
Notice that the strategies in round $T/2+1,...,T$ can be done only based on information from the first $T/2$ rounds. And also following Pandora's rule for agents in round $T/2+1,...,T$ will give no worse expected utilities for these agents. So $A(\sigma,T)$ will be no worse than the average utility of the above strategy.

On the other hand, for the above strategies, it's easy to see that for the first $T/2$ rounds, the expected utility is at least 0. In the last $T/2$, the expected utility will be at least  $\E[ \max(M(\sigma,T/2)-c, 0)]$. 

To sum up, we have $A(\sigma,T) \geq \E[ \max(M(\sigma,T/2)-c, 0 )]/2$.
\end{proof}

\begin{lemma}
\label{lem:qualitylb}
For any $h \geq 2 $ and $0 < \sigma < 1$, there exist large enough $T$ such that with probability at least $1/2$, $M(\sigma,T) \geq 4h + c$. 
\end{lemma}

\begin{proof}
Without loss of generality, we assume agents break tie by picking items with smaller numbers. 

Let $w = \frac{4 h + c + 2 }{(1- \sigma^2)^{3/2}}$ and $w' =\frac{4 h + c +2 }{(1-\sigma^2)\sigma}$ , we have $w, w' \geq 2$. Let's set $n$ to be  $6\sqrt{2\pi} w \cdot \exp(w^2/2)$. Then we have 
\begin{eqnarray*}
Pr\left[ \max(q_1,...,q_{n}) \leq \frac{4h + c + 2}{1-\sigma^2}\right] &=& \left(Pr\left[q_1 < \frac{4h + c+2}{1-\sigma^2}\right] \right)^{n}  \\
& =&  \Phi \left( \frac{4 h + c+2 }{(1- \sigma^2)^{3/2}} \right)^{n}.\\
&\leq& \left(1- \frac{\exp(-w^2/2)}{2\sqrt{2\pi} w}\right)^{n} \\
&\leq& \frac{1}{e^3} < 1/8.
\end{eqnarray*}

Define $W_t$ to be indicator function of the event that in round $t$, for all item $i \in [n]$, $q_i \leq \frac{4 h + c+2}{1-\sigma^2}$ implies $v_{i,t} < 0$. For any fixed $q_1,...,q_{n}$, 
\[
Pr[W_t = 1] \geq \left(Pr\left[s_{i,t} < -\frac{4 h + c+2}{1-\sigma^2}\right] \right)^{n} = \Phi(-w')^{n} \geq \frac{\exp(-(w')^2 n/2)}{2\sqrt{2\pi} \cdot w'}.
\]
Now we pick $T \geq 4\sqrt{2\pi} \cdot w'n  \exp((w')^2 n/2)$. Notice that $W_t$'s are independent after $q_i$'s are fixed. By Chernoff bound, we know that with probability at least $1-1/8$, $\sum_{t = 1}^{T} W_t \geq n$. 

By union bound, with probability at least $1-1/4$, we know $\exists i \in [n]$, $q_i > \frac{4 h + c+2}{1-\sigma^2}$ and $\sum_{t=1}^{T} W_t \geq n$. This implies an item $i \in [n]$ is explored after round $T$ with quality at least $\frac{4 h + c+2}{1-\sigma^2}$. 

Let $i^*$ be the item that has the highest quality among items $1,...,n$. Now consider the event that the empirical average value of $i^*$ is at least $q_{i^*} - 2\sigma$. By Lemma \ref{lem:gaussian}, we know this event happens with probability at least $1/4$. By union bound again, with probability at least $1-1/4-1/4 = 1/2$, item $i^*$ has empirical average value at least $\frac{4 h + c+2}{1-\sigma^2} - 2\sigma \geq \frac{4 h + c}{1-\sigma^2}$. Then by Fact \ref{fct:update} we have that, with probability at least $1/2$, $M(\sigma,T) \geq 4h + c$.
\end{proof}

Given these two lemmas, we set $n$ to be the same $n$ as in Lemma \ref{lem:qualitylb} and $T$ to be 2 times the $T$ in Lemma \ref{lem:qualitylb}. Then by Lemma \ref{lem:utilitylb} and Lemma \ref{lem:qualitylb}, 
\[
A(\sigma,T) \geq \E[ \max(M(\sigma,T/2)-c, 0 )]/2 \geq \frac{1}{2} \cdot (4h + c -c) \cdot \frac{1}{2} = h. 
\]


%------------------------------------------------------------------------------
%
%------------------------------------------------------------------------------














\subsection{Proof of Lemma \lowercase{\ref{lem:value}}}\label{sec:value_diamond}

The goal of this section is to show that $A(1,T)$ is at least $(1-o(1))D$ for $T = \omega(1/p)$. 

The proof has several technical considerations that did not appear in Lemma \ref{lem:diamonddiv} mainly because due to the more complicated behavior of agents. % as in Appendix \ref{sec:value}. 


Set $n=T$. When diversity level is 1, we have $\sigma = 1$. In this case $q_i = d_i$. For the proof, we consider the following procedure to sample the $q_i$ and $s_{i,t}$:
\begin{enumerate}[$\bullet$]
\item First sample each $q_i$ for $i = 1,...,n$.
\item Define $s'_{i,j}$ to be the subjective score of item $i$ when played the $j$-th time. For example, for agent $t$, when it chooses to observe item $i$ and this is the $j$-th time item $i$ is observed, then $s_{i,t} = s'_{i,j}$.
\item Sample $s'_{i,j}$ for $i=1,...,n$, $j = 1,...,T$. Notice that some of these $s'_{i,j}$'s might not be used.
\end{enumerate} 

We prove the following lemma to show that $\sum_{j=1}^J s'_{i,j}$ concentrates well. It is very similar to Lemma \ref{lem:gaussian}.

\begin{lemma}
\label{lem:dgaussian}
For any $\alpha \geq 2$, with probability at least $1 - \exp(-\alpha^2/2) \cdot \frac{1}{\alpha^2}$, for all $J = 1,...,T$, $\sum_{j=1}^J s'_{i,j}   < \alpha J $.
\end{lemma}
\begin{proof}

For each $J \in [T]$, 
\[
Pr\left[ \frac{\sum_{j=1}^J s'_{i,j}}{J} \geq\alpha \right] = 1 - \Phi\left(\alpha \sqrt{J}\right)  \leq \frac{1}{\sqrt{2\pi}} \exp(-\alpha^2J/2) \cdot \frac{1}{\alpha^2J} .
\]
The last inequality is by Fact \ref{fact:gaussiancdf}. Then by union bound, we have
\begin{align*}
Pr\left[ \max_{J \in [T]}\frac{\sum_{j=1}^J s'_{i,j}}{J} \geq \alpha \right] &\leq \sum_{J=1}^T \frac{1}{\sqrt{2\pi}} \exp(-\alpha^2J/2) \cdot \frac{1}{\alpha^2J} \leq \frac{2}{\sqrt{2\pi}} \exp(-\alpha^2/2) \cdot \frac{1}{\alpha^2} \\
&\leq \exp(-\alpha^2/2) \cdot \frac{1}{\alpha^2}. 
\end{align*}
\end{proof}

Let $m =\sqrt{ \min(T, 1/p^2) \cdot (1/p)}$. Since $n, T = \omega(1/p)$, we have $m = o( \min(T, 1/p^2) )$ and $m = \omega(1/p)$. Similarly as Lemma \ref{lem:utilitylb}, define $M(\sigma,T)$ to be maximum expected quality of all the items explored at the end of round $T$ conditioned on the history of $T$ rounds. Similarly as Lemma \ref{lem:utilitylb}, we have 
\[
A(1,T) \geq (1- m/T) \cdot \E[M(1,m) - c].
\]
In the rest of the proof we will just give a lower bound on $M(1,m)$.

Consider the following event $W$:
\begin{enumerate}[$\bullet$]
\item There exists $ i \in [m]$ such that $q_i = D$ (i.e. there's at least one diamond among the first $m$ items).
\item For all $i \in [m]$ such that $q_i = 0$,  $\sum_{j=1}^J s'_{i,j}   < J  \cdot \frac{D}{2}$, for all $J = 1,...,T$ .
\item For all $i \in [m]$ such that $q_i = D$,  $| \sum_{j=1}^J s'_{i,j} |   > -J  \cdot \frac{D}{3}$, for all $J = 1,...,T$.
\end{enumerate}

With Lemma \ref{lem:dgaussian}, $W$ happens with probability at least $1 - (1-p)^m - \exp(-D^2/18) \cdot \frac{18m}{D^2} = 1 - o(1)$. 

Now we start to study what items do agents explored in the first $m$ rounds condition on $W$. When agents use Pandora's rule, they will update distributions of $q_i$'s based on the history of observed values. Since $q_i$ can only be $D$ or $0$, each of these distributions can be described by one number meaning the probability of $q_i$ being $D$. Define $\theta_{i,t}$ to be the probability of item $i$ being $D$ conditioned on the history seen by agent $t$. 

We prove the following lemma about the Weitzman index. 

\begin{lemma}
\label{lem:dweitzman}
Let $x^*$ be the Weitzman index of an unobserved item. Assume before agent $t$, item $i$ has been observed $J>0$ times. 
\begin{enumerate}
\item If $q_i = 0$ and $\sum_{j=1}^J s'_{i,j}   < J  \cdot \frac{D}{2}$, the Weitzman index of item $i$ is smaller than $x^*$ for agent $t$.
\item If $q_i = D$ and $\sum_{j=1}^J s'_{i,j}   > -J  \cdot \frac{D}{2}$, the Weitzman index of item $i$ is larger than $x^*$ for agent $t$.
\end{enumerate}
\end{lemma}

\begin{proof}
First it's easy to see that the Weitzman index of item $i$ for agent $t$ is a monotone function of $\theta_{i,t}$, as the distribution of higher $\theta_{i,t}$ dominates the distribution of lower $\theta_{i,t}$. 

Let $\bar{v}$ be the average observed value of item $i$ before agent $t$. Notice that for iid Gaussian random variables, the average is the sufficient statistics. The agents calculate $\theta_{i,t}$ as following:
\[
\theta_{i,t} = \frac{p\cdot Pr[\sum_{j=1}^J s'_{i,j} /J= \bar{v} - D] }{p\cdot Pr[\sum_{j=1}^J s'_{i,j} /J= \bar{v} - D] + (1-p) \cdot Pr[\sum_{j=1}^J s'_{i,j}/J = \bar{v} ]\cdot }.
\]
When $\bar{v} = D /2$, since $Pr[\sum_{j=1}^J s'_{i,j} /J= \bar{v} - D] = Pr[\sum_{j=1}^J s'_{i,j}/J = \bar{v} ]$, we have $\theta_{i,t} = p$. When $\bar{v} > D/2$, we have $\theta_{i,t} > p$ and when $\bar{v} < D/2$, we have $\theta_{i,t} < p$. Since the Weitzman index of item $i$ for agent $t$ is a monotone function of $\theta_{i,t}$, we conclude the proof.
\end{proof}
Now we assume $W$ happens. We know that there is at least one item with $q_i = D$ among the first $m$ items. Assume the first such item has index $i^*$. By Lemma \ref{lem:dweitzman}, we know the explored items with $q_i = 0$ will have Weitzman index smaller than the Weitzman index of an unobserved item. Therefore before $i^*$ is explored, each agent we will explore one new item. So at the end of round $m$, item $i^*$ is explored. Define $\bar{v}$ to be the average value of item $i^*$. We know that conditioned on $W$, $2D/3 <\bar{v} < 4D/3$. As said in the proof of Lemma \ref{lem:dweitzman}, the agent calculates $\theta_{i^*,m}$ as the following (assuming item $i^*$ has been pulled $J$ times)
\[
\theta_{i^*,m} = \frac{p\cdot Pr[\sum_{j=1}^J s'_{i^*,j} /J= \bar{v} - D] }{p\cdot Pr[\sum_{j=1}^J s'_{i^*,j} /J= \bar{v} - D] + (1-p) \cdot Pr[\sum_{j=1}^J s'_{i^*,j}/J = \bar{v} ]\cdot }.
\]
Since $2D/3 <\bar{v} < 4D/3$, it is easy to check that the calculated $\theta_{i^*,m}$ will be at least $1 - \frac{1}{\exp(D^2/6) + 1}$. Then we have
\[
\E[M(1,m)] \geq Pr[W] \cdot (1 - \frac{1}{\exp(D^2/6) + 1}) D = (1-o(1)) D.
\]
To sum up, we get
\[
A(1,T) \geq (1- m/T) \cdot \E[M(1,m) - c] \geq (1-o(1))D.
\]





==> valuemodel_main.tex <==
%!TEX root =  main.tex

\section{Extension to ``Revealed Value'' Settings}
\label{sec:value_main}

%\jnote{To mix with the following two appendices}

In the ``revealed value'' model, agents only observe the total value the previous agents for the items they explored instead of learning exactly the decomposition in quality and subjective score. Agents infer the true quality using a Bayesian update rule. The inferred distribution of quality for an item is a Gaussian that depends on the average value that previous agents received as well as the number of them. The exact closed-form formula is given by Fact~\ref{fct:update}.

We revisit the settings we examined before in worlds with and without diamonds in the ``revealed value'' model.

\subsection{World without Diamonds}

Note that if the diversity level is 0, agents observe the exact same information and behave in the same way as in the ``revealed quality'' setting. Therefore Lemma \ref{lem:nodivub} holds in the value model as well. Similarly, when the diversity level is 1, agents behave the same as in the ``revealed quality'' as they still do not learn any information from previous agents. Therefore, Lemma \ref{lem:nodiv} also holds in the value model.

On the other hand, the behavior of agents under intermediate levels of diversity $\sigma \in (0,1)$ changes. However, similar to the ``revealed quality'' model, we show that intermediate levels of diversity $\sigma \in (0,1)$ can still be unboundedly better than extreme levels of diversity.

\begin{theorem}
\label{thm:value}
For any $\sigma \in (0,1)$, for large enough $T$, it holds that $A(1,T) \le A(0,T) \leq o(1) \cdot A(\sigma,T)$. 
\end{theorem}

The proof of Theorem~\ref{thm:value} is given in Appendix~\ref{sec:value} and follows by bounding the ``apparent'' quality of the best item explored after $T$ rounds. That is, in contrast to the case of ``revealed quality'', where we consider the true maximum quality after $T$ rounds, in this setting the  quantity of interest is the quality that an agent may infer about an item. This naturally captures the utility of the society as it quantifies the informational gain of the society at a given point.


\subsection{World with Diamonds}

In a world with diamonds, when the diversity level is $0$, agents behave again identically to the ``revealed quality'' case.
However, when the diversity level is 1, the behavior of agents changes. We show a fully diverse society can still benefit significantly by the existence of diamonds and we can prove that even in this case Lemma \ref{lem:diamonddiv} holds and thus we get that:

\begin{lemma}
\label{lem:value}
$A(0,T) = o(1) \cdot A(1,T)$ 
\end{lemma}

The proof requires showing that Lemma \ref{lem:diamonddiv} holds even in the revealed value setting and is presented in Appendix~\ref{sec:value_diamond}. 

